Group Surfing: A Pedestrian-Based Approach to Sidewalk Robot Navigation

In this paper, we propose a novel navigation system for mobile robots in pedestrian-rich sidewalk environments. Sidewalks are unique in that the pedestrian-shared space has characteristics of both roads and indoor spaces. Like vehicles on roads, pedestrian movement often manifests as linear flows in opposing directions. On the other hand, pedestrians also form crowds and can exhibit much more random movements than vehicles. Classical algorithms are insufficient for safe navigation around pedestrians and remaining on the sidewalk space. Thus, our approach takes advantage of natural human motion to allow a robot to adapt to sidewalk navigation in a safe and socially-compliant manner. We developed a \textit{group surfing} method which aims to imitate the optimal pedestrian group for bringing the robot closer to its goal. For pedestrian-sparse environments, we propose a sidewalk edge detection and following method. Underlying these two navigation methods, the collision avoidance scheme is human-aware. The integrated navigation stack is evaluated and demonstrated in simulation. A hardware demonstration is also presented.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> Text/case_study.tex <==

To demonstrate the navigation system in the real world, we have set up a case study on our university campus. The goal of this study is to autonomously navigate a sidewalk robot from our lab to a local coffee shop and back. On a well populated sidewalk, the robot will have to share the space with pedestrians walking both towards and away from the goal and must correctly imitate groups to cross an intersection. At times where pedestrians are sparse, the robot must switch successfully to the sidewalk edge detection method for navigation. Throughout the demonstration, the robot must also successfully avoid any collisions with both static and dynamic objects on the sidewalk. 
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:58:08.243Z:
%
% > The goal of this study is to autonomously navigate a sidewalk robot from our lab to a local coffee shop and back
%
% ^.

\begin{figure}[H]
\centering   
\subfigure[]{\label{fig:a}\includegraphics[width=.45\textwidth]{images/map.png}}
\subfigure[Simplified simulation environment of the region in figure \textbf{a}.]{\label{fig:b}\includegraphics[width=.45\textwidth]{images/caris_model.png}}
\caption{A user sets a pick up destination on a map browser application. The robot GPS location is used to display the robot's current location.}
\end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[width=\textwidth]{images/google_map.png}
%         \caption{A user set a pick up destination on a map browser application. It displays the GPS way-point trajectory and the current robot location.}
%         \label{fig:gull}
%     \end{subfigure}
%      \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[width=\textwidth]{tiger}
%         \caption{A tiger}
%         \label{fig:tiger}
%     \end{subfigure}~
%     \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[width=\textwidth]{mouse}
%         \caption{A mouse}
%         \label{fig:mouse}
%     \end{subfigure}
%     \caption{Pictures of animals}\label{fig:animals}
% \end{figure}


==> Text/old.tex <==
% NJH
Existing dynamic collision-avoidance approaches are either model-based, learning-based, or a combination thereof. Model-based approaches require an accurate and general mathematical model, which is both difficult to develop and expensive to compute online. Learning-based approaches, while difficult and time-consuming to train offline, offer a more generalizable result and are less expensive online. \cite{Kruse13}

Human-aware behaviours can be induced in either family of collision-avoidance approaches. Socially-aware behaviours, such as pedestrian conventions and appropriate proxemics, can be induced through either cost functions in model-based approaches, or reward functions in reinforcement learning-based approaches.
\cite{Kruse13}

==> Text/related_work.tex <==
Augmented Reality (AR) is a promising alternative for industry, It facilitates interaction by enhancing the physical world with virtual computer generated information~\cite{azuma1997survey}. Assembly~\cite{wang2016comprehensive}, training~\cite{webel2013augmented}, maintenance~\cite{engelke2015content} and repair~\cite{henderson2011exploring} have been some of the industrial activities that researchers have explored using AR.

Merging AR with robotic systems bring new HRI possibilities.
For instance~\cite{fang2014novel}~\etal prosed an AR interface that uses a marker-cube attached with a probe that allows the user to guide a virtual robot by setting way-points and orientations. The AR scene was visualized through a monitor. The authors pointed out that participants tented  to focus on the screen more than on the real scenario and because depth is difficult to perceive from the display it turns into improper guidance of the robot. An important component for an effective HRI is the share space between human and robot~\cite{breazeal2001active}. 




% Recently 
% The Hololens~\cite{kress201711} is the first untethered mixed reality head-mounted display that allows holographic visualization. It has multiple CPU's, a holographic processor unit, a depth camera, five RGB cameras, an inertial measurement unit, microphone and speakers. Its SDK support functionalities like gaze tracking, basic hand gesture recognition, spatial sound, voice recognition and using sensor fusion techniques is capable of map its surrounding and allow interaction between the real and virtual world, while tracking the users head pose. 





~\cite{breazeal2001active}
"One of the key
requirements that have been identified for effective HRI is
the overlapping space that can be perceived by both the
human user and the robot programming system 





Meanwhile, the participants tended
to focus on the monitor’s view when performing the tasks.
This will to some extent lead to improper guidance of the
virtual robot as it is not easy for the operator to perceive the
depth information from the display on the monitor.

hen displaying feedback on a screen that is located next to
where the actions are performed, users have to transfer the
information that is shown on a screen to the real world. This
requires cognitive effort and consumes time.


allows to specify for program interactive robot path and end-effector orientation planning of a virtual robot. 



. An ARToolKitbased
tracking method is adopted for tracking a handheld
device, which is a marker-cube attached with a probe, and virtual
robot registration. The tracked interaction device allows
the users to interact with spatial information of the working
environment. It can be used to guide the virtual robot to intervene
in the path planning and end effector (EE) orientation
planning processes. The actual working environment, the virtual
robot model, the trajectory information, as well as the
interaction processes are visualized through a monitor-based
display





Meanwhile, the participants tended
to focus on the monitor’s view when performing the tasks.
This will to some extent lead to improper guidance of the
virtual robot as it is not easy for the operator to perceive the
depth information from the display on the monitor.


A virtual robot is visualize in the real world through a monitor. The virtual robot is program by using a marker cube and some 



For instance Ni \etal~\cite{ni2017haptic} propose an off-line trajectory programming of a remote robot by using an AR interface for selecting candidate welding points in a remote location. Using a phantom haptic device The user teleoperate through a monitor a virtual robot that is overlay on the remote scene using markers. 






Merging AR with a robotics provides new ways to interact with a robot system. 




For instance Hanson \etal~\cite{hanson2017augmented} study the use of AR to instruct an operator to preassemble individual items into ready-to-ship kit and compare it with paper list method. They report that AR is competitive both in terms of
time-efficiency and picking accuracy

completing a kit by picking different parts from a set of bins. Their study shows that task performance was improved in comparison with current methods.


Merging AR with robotic systems provides new ways to interact with a robot system. 

During this exploration, researchers have found that collocation of the information is 


Merging AR with robotic systems provides new ways to interact with a robot system.  



As point out by different researchers 
We learned that good feedback
should fulfill two requirements: it should be displayed directly
at the position where an action is required, and displayed feedback should be context-aware to match the performed actions.
When displaying feedback on a screen that is located next to
where the actions are performed, users have to transfer the
information that is shown on a screen to the real world. This
requires cognitive effort and consumes time.


An interface for interactive robot path and end-effector orientation planning is proposed by Fang \etal. Where a virtual robot is visualize in the real world through a monitor. The virtual robot is program by using a marker cube and some 


~\cite{fang2014novel}
Meanwhile, the participants tended
to focus on the monitor’s view when performing the tasks.
This will to some extent lead to improper guidance of the
virtual robot as it is not easy for the operator to perceive the
depth information from the display on the monitor.



For instance Ni \etal~\cite{ni2017haptic} propose an off-line trajectory programming of a remote robot by using an AR interface for selecting candidate welding points in a remote location. Using a phantom haptic device The user teleoperate through a monitor a virtual robot that is overlay on the remote scene using markers. 

When the user get close to the welding surface a force feedback help users maintain a constant distance from the workpiece surface. Orientation and location are store by pressing a button in the haptic device.Then the recorded welding candidate points are used to fit as a curve for programming the real welding robot.





Haptic and visual augmented reality interface for programming welding robots









For each part number that should be picked, a discreet
yet clearly visible virtual 3D “tunnel” guided the picker to the
right bin. When the bin was within the picker’s field of view, a coloured
circle and a number would appear in the bin, indicating how many
components should be picked of the part number in question






and have experimentally shown that 






In particular AR 


The common space that is share by the user and the robot programming system 





~\cite{breazeal2001active}
"One of the key
requirements that have been identified for effective HRI is
the overlapping space that can be perceived by both the
human user and the robot programming system 




Improve the performance, reduce errors and reduce cognitive load of industrial operators. 





For instance Andersen \etal ~\cite{andersen2016projecting} created an interface based on projections on a physical surface to visualize robot task information and intentions during a car door assembling task. Some limitations of there system includes occlusion of the information by the humans in the scene and no human tracking.  






~\cite{breazeal2001active}
"One of the key
requirements that have been identified for effective HRI is
the overlapping space that can be perceived by both the
human user and the robot programming system [4].
"--> Breazeal C, Edsinger A, Fitzpatrick P et al (2001) Active vision
for sociable robots. IEEE Trans Syst Man Cybern A
31(5):443–453


As point out by different researchers 
We learned that good feedback
should fulfill two requirements: it should be displayed directly
at the position where an action is required, and displayed feedback should be context-aware to match the performed actions.
When displaying feedback on a screen that is located next to
where the actions are performed, users have to transfer the
information that is shown on a screen to the real world. This
requires cognitive effort and consumes time.





The actual working environment,
the virtual robot model, the trajectory information,
as well as the interaction processes are visualized
through a monitor-based display.



Chong
et al. [43] presented an interface through which the users could
guide a virtual robot using a probe attached with a single marker.
Fang et al. [44] improved this HRI interface through which the
user could interact with the spatial environment using a markercube
based interaction device. Zaeh and Vogl [8] introduced a
laser-projection-based approach where the operators could
manually edit and modify the planned paths projected over a
real workpiece using an interactive stylus.





 In VR the visual capture~\cite{welch2013perceptual} effect may reduce the error sensation from the user's point of view. This effect is the tendency of the brain to believe what it sees rather than what it feels, hears, and so on. That is, visual information tends to override all other senses. 
In contrast in AR Registration errors result in visual-visual conflicts between the images of the virtual and real hands


Augmented reality demands much more accurate registration
than do virtual environments (Azuma, 1993).
Imagine the same scenario of a user holding up her
hand, but this time wearing a see-through HMD. Registration
errors now result in visual-visual conflicts between
the images of the virtual and real hands.








% *Common ground between robot and human--common knowledge.
% **Understand internal states of the robot


% Insitu interfaces. Directly talk with the robot? use a external device to interact a tablet, phone etc. 
% Direct interface speech , gestures etc. 
% *AR bring both collocation and extra information to define a task 
% **We argue that collocation improves understanding of the process 





% *Preview of the motion




% VIBI
% Chiorcale
% inside a vr world to control robot
% pointing gestures

% Different type of interfaces:: 

% Remote interfaces: User in a different location. 

% Stream images, point clouds, merge with 3d models etc. 







% Understanding robot


% lated research studies have focused on providing a visual
% platform for human users to directly interact and understand
% the internal states of robots.


==> Text/system_old.tex <==
\begin{figure}[H]
\centering
\includegraphics[width=.4\textwidth] {images/System_Overview.jpg}
\caption{High-level overview of our proposed system}
\label{fig:system_overview}
\end{figure}
The block diagram of our proposed system is shown in Figure ~\ref{fig:system_overview}. This system allows a user to specify a delivery destination that is executed by a robotic mobile platform that navigates along sidewalks. This is done by having the user interacting with a map browser to select a pick-up location. Such information is then utilized by control module and fed to navigation module. In the meantime, sensing module provides the necessary information to both control and navigation modules. Ultimately, velocity command from the navigation module will be used to move the robot.
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:51:48.942Z:
%
% > will be used
%
% ^.
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:51:38.087Z:
%
% ^.
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:51:30.767Z:
%
% ^.
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:51:03.364Z:
%
% > Such
%
% ^.
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:50:49.406Z:
%
% > This is done by having the user interacting
%
% ^.

% Can all of us look through this part (sensing)? % 
\subsection{Sensing}
Our mobile robot is equipped with multiple sensors: GPS, IMU, a VLP-16 - Velodyne LiDAR 3D laser Sensor, a SICK LMS-200 2D laser sensor and a Realsense RGB-D sensor. The sensing module is in charge of providing the control module and the navigation module the necessary data to navigate in the real world. The GPS and the IMU will be used by the control module to determine both the current position and orientation of the robot. In the navigation module, the RGB-D sensor is used to track pedestrian while the 3D laser sensor is used to detect sidewalk. %CP: this is not completely true in simulation we used the velodyne to find legs and we are not using the rgbd sensor. 
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:52:37.121Z:
%
% > GPS, IMU, a VLP-16 - Velodyne LiDAR 3D laser Sensor, a SICK LMS-200 2D laser sensor and a Realsense RGB-D sensor. 
%
% ^.
Obstacle avoidance is achieved by using the information from the 2D laser sensor.

\subsection{Control}

The control module is in charge of translating user's input into local subpoint that is used by the navigation module to move the robot. The initial position and orientation of the robot is first obtained. After the user selects a global goal $G$ (pick-up location), a path is computed by Google Maps' API with waypoints $W_n$ located at each intersections from the robot's initial location to the goal, see Figure \ref{fig:goal_selection}. Even though these waypoints are inaccurate for sidewalk navigation, as the average error is $\pm7m$ after multiple sampling across our campus, they can be used as a coarse estimate of what direction to move on the sidewalk. Using the next waypoint, a local subpoint short distances away from the robot is then calculated to be used as directional guidance for the navigation module. Depending on whether there is any pedestrian moving towards the local subpoint, the local subpoint will be send to either \textbf{Group Surfing} or \textbf{Sidewalk Following} of the navigation module. Simultaneously, the control module will also check for arrival of the robot at the waypoint by measuring the difference in distances between the robot and the next waypoint and comparing it to goal tolerance. If the distance is smaller than the goal tolerance, then the robot is assumed to be arrived at the waypoint. If there is any remaining waypoints left, the subsequent waypoint will be used to obtain a local subpoint and the process loops until the robot reaches the final waypoint. The control module is done in state machine as shown in Figure ~\ref{fig:control_module}.
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:53:43.926Z:
%
% > be
%
% ^.
% * <elizabeth.croft@ubc.ca> 2018-08-20T12:53:31.971Z:
%
% >  will be send
%
% ^.

\begin{figure}[H]
\begin{tikzpicture}[scale=1.25]
\centering
	% Draw robot
    \draw (1,1) node[rectangle,fill,inner sep=5pt,label=below:$R$, rotate=30](){};
    
    % Draw global goal, waypoints and subpoint
    \draw[dotted] 
    	(1,1) node[] (Initial Position){}
      -- (3.5,2.5) 
      	node[diamond,fill=red,inner sep=1.5pt,label=above:$W_1$] (){}
        node[circle,dashed,draw=black,thick,inner sep=5pt] (){}
      	node[pos=.25,circle,fill,inner sep=1pt,label=above:$S$] (){} 
      -- (4.3,1.3) 
      	node[diamond,fill=red,inner sep=1.5pt,label=below:$W_2$] (){}
        node[circle,dashed,draw=black,thick,inner sep=5pt] (){}
      -- (7,3) 
      	node[star,star points=6,fill=blue,inner sep=2pt,star point ratio=2,label=below:$W_3$,label=above:$G$] (){}
        node[circle,dashed,draw=black,thick,inner sep=5pt] (){};
      
    %Draw robot direction
    \draw[->,color=black,] (1,1) -- ++(.5,.3);

\end{tikzpicture}
\caption{Distinction between global goal $G$, waypoints $W$ and subpoint $S$. Dashed circles resemble goal tolerance for the robot to be considered arrived.}
\label{fig:goal_selection}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=.5\textwidth] {images/Control_Module.jpg}
\caption{Control module}
\label{fig:control_module}
\end{figure}

\subsection{Navigation}
The navigation module is in charge of moving the robot towards the local subpoint while avoiding any obstacle in the way. To achieve local sidewalk navigation, we introduce a \textbf{Group Surfing} approach which relies on nearby pedestrian flow on the sidewalk for autonomous robot navigation. Group surfing is our default navigation mode and our system expects to find humans walking on sidewalks. However, in case where no humans are present, we have developed a contextual approach method which is \textbf{Sidewalk Following} to estimate the boundary between the sidewalk and street and propose a estimate local goal for navigation. During Group surfing or Sidewalk Following, \textbf{Collision Avoidance} is active. These three methods are explained in detail in Section \ref{sec:Methods}.

\begin{figure}[H]
\centering
\includegraphics[width=.4\textwidth] {images/Navigation_Module.jpg}
\caption{Navigation module}
\label{fig:navigation_module}
\end{figure}

%interconnected modules: sensing, planning, and reacting. %The sensing component uses a 2D laser scan input and a %RGB-D sensor input to track humans, the sidewalk curb, %and any other obstacles. The planning component uses the %robot's current GPS location and coordinates for a goal %to compute a path with waypoints at each intersection. %Both these components output to the Reacting component, %which enacts local planning to reach each waypoint in a %safe manner.

% in conjunction with the sensing module to select a navigation strategy during execution. 

% Our navigation system is composed of

% The navigation component uses the robot's current GPS location and coordinates for a goal to compute a path with waypoints at each intersection. Both these components output to the Reacting component, which enacts local planning to reach each waypoint in a safe manner.
% \subsection{Navigation behaviour}
% As the novel contribution of our system lies in the ability to 'group surf' by moving along with pedestrian groups, there must also be an alternate navigation method when pedestrians are too sparse. The chosen navigation behaviour of the robot depends on a continuous analysis of whether there are groups on the sidewalk moving towards the waypoint. If not, the system falls back to following along the curb of the sidewalk. Given either local subgoal, the planner provides a path to the subgoal that will avoid any static or dynamic obstacles, such as other pedestrians. Upon reaching each subgoal, the system scans for pedestrians and the navigation behaviour loops until reaching each waypoints and ultimately the global goal, as shown in Fig. \ref{fig:block_diagram}.

% a goal selection system computes the optimal navigable path to this global goal. This path which lies along sidewalks has waypoints at each intersection. Between the waypoints are incremental points $S_n$ that are used as goals for the lower level group-following or curb-following controllers. Upon reaching each $S_n$, the goal selection system will internally update the position and orientation of the robot and subsequently mitigate the accumulation of location errors of the GPS.
 
 %Control module 
  
%  Using the interface module the user specify a delivery from point A to B using a browser interface, where the current location of the robot is display and a origin and destination can be set by the user.



%\subsection{System overview}
% System Block Diagram Figure, needs to be updated to incorporate curb detection


% \begin{figure}[]
% \centering
% \includegraphics[width=.45\textwidth] {images/System_Overview.png}
% \caption{Block diagram overview of the proposed navigation system}
% \label{fig:block_diagram}
% \end{figure}

% \subsection{Goal selection}

% With a global goal as a user's input and the initial position and orientation of the robot as internal inputs, the goal selection system computes the optimal navigable path to this global goal. This path which lies along sidewalks has waypoints at each intersection. Between the waypoints are incremental points $S_n$ that are used as goals for the lower level group-following or curb-following controllers. Upon reaching each $S_n$, the goal selection system will internally update the position and orientation of the robot and subsequently mitigate the accumulation of location errors of the GPS.

%Do we need this figure still??
%\begin{figure}[H]
%\centering
%\includegraphics[width=.4\textwidth] {images/Nav_Behaviour_Flowchart.png}
%\caption{Navigation behaviour flowchart}
%\label{fig:block_diagram}
%\end{figure}

